LDP-FL: Practical Private Aggregation in Federated Learning with Local Differential Privacy

Train machine learning models on sensitive user data has raised increasing privacy concerns in many areas. Federated learning is a popular approach for privacy protection that collects the local gradient information instead of real data. One way to achieve a strict privacy guarantee is to apply local differential privacy into federated learning. However, previous works do not give a practical solution due to three issues. First, the noisy data is close to its original value with high probability, increasing the risk of information exposure. Second, a large variance is introduced to the estimated average, causing poor accuracy. Last, the privacy budget explodes due to the high dimensionality of weights in deep learning models. In this paper, we proposed a novel design of local differential privacy mechanism for federated learning to address the abovementioned issues. It is capable of making the data more distinct from its original value and introducing lower variance. Moreover, the proposed mechanism bypasses the curse of dimensionality by splitting and shuffling model updates. A series of empirical evaluations on three commonly used datasets, MNIST, Fashion-MNIST and CIFAR-10, demonstrate that our solution can not only achieve superior deep learning performance but also provide a strong privacy guarantee at the same time.

==> 11-abstract.tex <==
\begin{abstract}
Training deep learning models on sensitive user data has raised increasing privacy concerns in many areas. Federated learning is a popular approach for privacy protection that collects the local gradient information instead of raw data. One way to achieve a strict privacy guarantee is to apply local differential privacy into federated learning. However, previous works do not give a practical solution due to three issues. First, the noisy data is close to its original value with high probability, increasing the risk of information exposure. Second, a large variance is introduced to the estimated average, causing poor accuracy. Last, the privacy budget explodes due to the high dimensionality of weights in deep learning models and many query iterations of federated learning. In this paper, we proposed a novel design of local differential privacy mechanism for federated learning to address the abovementioned issues. It is capable of making the data more distinct from its original value and introducing lower variance. Moreover, the proposed mechanism bypasses the curse of dimensionality by splitting and shuffling model updates. A series of empirical evaluations on three commonly used datasets, MNIST, Fashion-MNIST and CIFAR-10, demonstrate that our solution can not only achieve superior deep learning performance but also provide a strong privacy guarantee at the same time. 
\end{abstract}

%The proposed mechanism achieves a privacy budget of $\epsilon=1$ with 0.97\% accuracy loss on MNIST, a privacy budget of $\epsilon=4$ with 1.32\% accuracy loss on Fashion-MNIST, and a privacy budget of $\epsilon=10$ with 1.09\% accuracy loss on CIFAR-10, respectively

% In this paper, we proposed a new local differential privacy mechanism that makes data more distinct to its original value and introduces lower variance, which achieves the state-of-the-art performance within a small privacy cost $\epsilon$.
% Moreover, our solution bypasses the curse of dimensionality by splitting and shuffling model updates.
% A series of empirical evaluations show that our solution can not only achieve a superior performance but also provide a strong privacy guarantee.
% For example, on MNIST, the central model trained by our system can achieve privacy $\epsilon=1$ with merely 0.97\% accuracy loss. Moreover, experiments on CIFAR-10 achieve $\epsilon=10$ with 1.99\% accuracy loss. 

==> 12-body.tex <==
\section{Introduction}


Many attractive applications involve training models on highly sensitive data, to name a few, diagnosis of diseases with medical records, or genetic sequences~\cite{alipanahi2015predicting}.
In order to protect the privacy of the training data, various privacy protection works have been proposed in the literature \cite{ma2018pdlm,michie1994machine, nissim2007smooth, samangouei2018defense}. 
The federated learning framework is of particular interest since it can provide a well-trained model without touching any sensitive data directly \cite{konevcny2016federated,mcmahan2016communication}.
The original purpose of the federated learning framework is to share the weights of the model trained on sensitive data instead of data directly.
However, some studies show that the weights also can leak privacy and recover the original sensitive data \cite{papernot2017semi}.
In order to solve the problem, recent works start to use differential privacy to protect the private data in federated learning \cite{bhowmick2018protection,geyer2017differentially,nguyen2016collecting}, but most of them can not give a practical solution for deep learning on complex dataset due to the trade-off between privacy budget and performance.

In previous approaches, there are several apparent concerns and challenges. First, the noisy data is close to its original value with high probability, increasing the risk of information exposure. For example, the price of a pen is 5. After data perturbation, the protected information is close to 5, such as 5.3, still leaking information. Second, a large variance is introduced to the estimated average, causing poor accuracy. As a result, it requires more communication between the cloud and clients for the learning convergence. Third, the privacy budget explodes due to the high dimensionality of weights in deep learning models. Last, to the best of our knowledge, no existing works have shown an excellent deep learning performance on popular datasets such as MNIST \cite{lecun2010mnist}, Fashion-MNIST \cite{xiao2017fashion} and CIFAR-10 \cite{krizhevsky2009learning},  with a reasonably small privacy budget.

%=====================================================
\begin{figure*}[tb]
\centering
\includegraphics[width=5.4in]{figures/NIPS20-LDP-1.pdf}
\caption{The overview of \system. Each client has a private dataset. After training their model locally, clients perturb their model weights with differentially private noise, and locally split and shuffle the weights to make them less likely to be linked together by the cloud. Finally, they send the weights to the cloud for aggregation.} \label{fig:framework}
\end{figure*}
%======================================================

In this paper, we proposed Locally Differential Private Federated Learning (\system), a new local differential privacy (LDP) mechanism to solve the above issues. As shown in Fig. \ref{fig:framework}, novelly designed local data perturbation and local model weights splitting and shuffling are applied to a typical federated learning system. 

Our main contribution is multifold. First, we propose a new LDP mechanism, and show how to apply it to federated learning. We prove our LDP mechanism is securer than existing mechanisms with a much reduced risk of information exposure by making the perturbed data more distinct from its original value.
Second, we apply splitting and shuffling to each clients' gradients to mitigate the privacy degradation caused by high data dimension and many query iterations. Third, we prove that our solution introduces less variance to average calculation, making it capable of presenting a better model training performance.
Last, we evaluate \system\ on three commonly used dataset in previous works, MNIST \cite{lecun2010mnist}, Fashion-MNIST \cite{xiao2017fashion} and CIFAR-10 \cite{krizhevsky2009learning}. 
The proposed mechanism achieves a privacy budget of $\epsilon=1$ with 0.97\% accuracy loss on MNIST, a privacy budget of $\epsilon=4$ with 1.32\% accuracy loss on Fashion-MNIST, and a privacy budget of $\epsilon=10$ with 1.09\% accuracy loss on CIFAR-10, respectively.
To our best knowledge, this work gives the first practical LDP solution for federated deep learning with a superior performance.
%Under similar conditions, Bhowmick et. al.  \cite{bhowmick2018protection} achieves weaker privacy with $\epsilon=500$ for MNIST and $\epsilon=5000$ for CIFAR-10.



%which has the limitation that the noisy data is close to its original value with high probability, increasing 

%First, we show how to use LDP to protect federated learning by the proposed data perturbation with theoretical guarantees.
%Second, we well discussed the different mechanisms to do the LDP and the difference between traditional differential privacy and LDP in federated learning.
%Third, we not only give the new theoretical analysis of the proposed framework but also first provide a practical solution that supports the LDP can protect the privacy of the gradient updating and the performance of the model.

% move the below here (was before "our main contribution".

 

%each weight update of a client needs to be perturbed to protect the data privacy.
%Unlike previous approaches, we apply splitting and shuffling for each client's weight updates.
%The cloud is still able to accurately estimate the average of the perturbed gradients from all clients and send the updated new gradient to each client for the next iteration.

% In our solution, clients do not need to trust each other or the cloud.
% As per the definition of LDP, it protects a user's all the data. Notice here ``user'' refers to who generates or owns the data, not necessarily the client. The client may have multiple users' data. For instance, a hospital is a client, and a sub-dataset is one patient's data. 
%Making the client's data indistinguishable requires adding a lot of noise and would profoundly affect the performance of federated learning. As LDP only needs each user's data to be indistinguishable, the client may partition its data into multiple sub-datasets, calculate gradients and add noises on each sub-dataset then sends all noisy gradients to the cloud.






\section{Preliminary}
%In this section, we briefly review the definitions of LDP and federated learning.

% \subsection{Differential Privacy}

% To satisfy the increasing demand for preserving privacy, differential privacy (DP) \cite{10.1007/11681878_14} was proposed as a rigorous principle that guarantees provable privacy protection and has been extensively applied %in both industrial and academic settings
% \cite{Andres:2013,friedman2010data,apple_dp}. 

% Let $f$ be a deterministic function that maps the dataset $D$ to the real numbers $\mathbb{R}$. 
% This deterministic function $f$, under the context of differential privacy, is called a query function of the dataset $D$.
% For example, the query function may request the mean of a feature in the dataset, the gender of each sample.
% The goal in privacy is to ensure that when the query function is applied on a different but close dataset $D'$, the outputs of the query function are indistinguishably comparing to that from the dataset $D$ such that the private information of individual entries in the dataset can not be inferred by malicious attacks.
% Here, two datasets $D$ and $D'$ are regarded as adjacent datasets when they are identical except for one single item.
% % Informally speaking, a randomized data release mechanism for a query function $f$ is said to ensure DP if  ``neighboring'' inputs induce similar distributions over the possible outputs of the mechanism. 
% % DP is particularly useful for quantifying privacy guarantees of queries computed over a database with sensitive entries. 
% The formal definition of differential privacy is given below.


% \begin{definition}[Differential Privacy {\cite[Definition~2.4]{dwork2011a}}]
% A randomized mechanism $\mathcal{M}$ is $(\epsilon, \delta)$-differentially private if for any adjacent dataset $D$, and $D'$, i.e $\|D-D'\|_1 \leq 1$, and any output $Y$ of $\mathcal{M}$, we have
%   \begin{equation}
%     \Pr [\mathcal{M} (D) = Y] \le {e^\epsilon } \cdot \Pr [\mathcal{M} (D') = Y]+\delta. 
%   \end{equation}
% \end{definition}
% If $\delta = 0$, we say that $\mathcal{M}$ is $\epsilon$-differentially private.
% The weight $\epsilon$ represents the privacy budget~\cite{dwork2011differential} that controls the privacy loss of $\mathcal{M}$. 
% A larger value of $\epsilon$ indicates weaker privacy protection.

% \begin{definition}[Differential Privacy {\cite[Definition~2.4]{dwork2011a}}]
% A randomized mechanism $\mathcal{M}$ is $(\epsilon, \Delta^S)$-differentially private if for any adjacent data $D$ and $D'$, i.e $\|D-D'\|_1 \leq 1$, and any output $Y$ of $\mathcal{M}$, we have
%   \begin{equation}
%     c(o; \cM, aux, D, D') \triangleq \log \frac{\Pr[\cM(aux, D) = o]}{\Pr[\cM(aux, D') = o]},
%   \end{equation}
% \end{definition}
% The privacy loss random variable $C(\cM, aux, D, D')$ is defined as $c(\cM(d); \cM, aux, D, D')$, i.e. the random variable defined by evaluating the privacy loss at an outcome sampled from $\cM(D)$.


% From the notion of the DP, we know the sensitivity of the deterministic function $f$ (i.e. a query function) regarding the dataset is important for designing the mechanism for the query function.
% For different noise mechanisms, it requires different sensitivity estimation.
% % In previous study of differential private deep learning, all mechanisms used the classical sensitivity analysis, named  ``\textbf{Global sensitivity}''.
% For example, the $\ell_2$-norm sensitivity $\Delta_2 f$ of the query function $f$ is used for Gaussian mechanism which is defined as $\Delta_2 f = \max_{D,D'}\left\| {f(D) - f(D')} \right\|_2$, where $D$ and $D'$ are two neighboring datasets.
% For the Laplacian mechanism, it uses the $\ell_1$-norm sensitivity $\Delta f$ for random noise sampling.
% In essence, when the sensitivity is smaller, it means that the query function itself is not very distinguishable given different datasets.


% A general method for enforcing a query function $f$ with the $(\epsilon,\delta)$-differential privacy is to apply additive noise calibrated to the sensitivity of $f$. 
% A general method for conveniently ensuring a deterministic query $f$ to be the $(\epsilon,\delta)$-differential privacy is via perturbation mechanisms that add calibrated noise to the query's output \cite{dwork2014algorithmic, dwork2010boosting, nissim2007smooth, duchi2013local}. 

% \begin{thm}[\cite{dwork2014algorithmic}]\label{thm:laplacian}
% If the $\ell_1$-norm sensitivity of a deterministic function $f$ is $\Delta^S f$, we have:
%     \begin{equation}
%     \mathcal{M}_f (D) \triangleq f(D)+Lap(\frac{\Delta f}{\epsilon} ),
%     \end{equation}
% where $\cM_f$ preserves $(\epsilon, 0)$-differential privacy, and $Lap(b)$ is the Laplacian distribution with location $0$ and scale $b$.
% \end{thm}


% \begin{thm}[\cite{dwork2014algorithmic}]\label{thm:gaussian}
% If the $\ell_2$-norm sensitivity of a deterministic function $f$ is $\Delta _2 f$, we have:
%     \begin{equation}
%     \mathcal{M}_f (D) \triangleq f(D)+\mathcal{N}(0, {\Delta_2 f}^2\sigma^2),
%     \end{equation}
% where $\mathcal{N}(0, {\Delta_2 f}^2\sigma^2)$ is a random variable obeying the Gaussian distribution with mean 0 and standard deviation ${\Delta_2 f}\sigma$. The randomized mechanism $\mathcal{M}_f(D)$ is $(\epsilon,\Delta)$ differentially private if $\sigma  \ge \sqrt {2\ln (1.25/\Delta )} /\epsilon $ and $\epsilon < 1$.
% \end{thm}


% A general method for approximating a deterministic function $f$ with $\epsilon$-differential privacy is to add noise calibrated to the global sensitivity of $f$, denoted as $\Delta f$, which is the maximal value of ${\left\| {f(x) - f(x')} \right\|}$ among any pair of $x$ and $x'$. For instance, the Laplacian mechanism is defined by,
% \begin{equation}
% \mathcal{M}_f (x) = f(x)+Lap(\frac{{\Delta f}}{\epsilon }),
% \end{equation}
% where $Lap(\frac{{\Delta f}}{\epsilon })$ is a random variable sampled from the Laplace distribution with scale $\frac{{\Delta f}}{\epsilon}$.

\subsection{Local Differential Privacy}

%In differential privacy, it is required to trust the party to collect the data and apply the necessary noise. However, such trust is not always feasible in many applications. Therefore, a recent concept of differential privacy was  tailored to the privacy-preserving data analysis. 
% It aims at providing provable privacy guarantee for each sensitive data sample, unlike general differential privacy is protecting the whole sensitive dataset \cite{Beimel2014}. 
Formally, the definition of $\epsilon$-LDP is given as below:

\begin{definition}~\cite{dwork2011differential}
  A randomized mechanism $\mathcal{M}$ satisfies $\epsilon$-LDP, for any pair input $x$ and $x'$ in $D$, and any output $Y$ of $\mathcal{M}$,
  \begin{equation}
    \Pr [\mathcal{M} (x) = Y] \le {e^\epsilon } \cdot \Pr [\mathcal{M} (x') = Y].
  \end{equation}
\end{definition}
where the inputs $x$ and $x'$ are any two inputs.
The privacy guarantee of mechanism $\mathcal{M}$ is controlled by privacy budget \cite{dwork2011differential}, denoted as $\epsilon$.
A smaller value of $\epsilon$ indicates a stronger privacy guarantee. 
%According to this definition, a local differentially private algorithm can provide aggregate representations about a set of data items without leaking information of any data item.

% The moments accountant enjoys good properties of composability and tail bound as given in~\cite{abadi2016deep}:

\textbf{\emph{[Composability]}}~\cite{abadi2016deep}. 
Suppose that a mechanism $\cM$ consists of a sequence of adaptive mechanisms $\cM_1, \ldots, \cM_k$,
    where $M_i: \prod^{i-1}_{j=1} \cR_j \times \cD \rightarrow \cR_i$. 
Then, for any $\lambda$
\[{\alpha _\cM}(\lambda ) \le \sum\limits_{i = 1}^t {{\alpha _{{\cM_i}}}(\lambda )}.\]
where $\alpha_{\cM}$ is conditioned on $\cM_i$’s output being $o_i$ for $i < t$.

By using the composability property, we can bound the moments of randomized mechanism based on each sub-mechanism, and then convert the moments accountant to $\varepsilon$-local differential privacy based on the tail bound.

The immunity to post-processing \cite{dwork2014algorithmic} also works on LDP, which claims no algorithm can compromise the differentially private output and make it less differentially private. 


\subsection{Federated Learning}

Federated learning \cite{mcmahan2016communication,konevcny2016federated} has been proposed and widely used in different approaches.
The motivation is to share the model weights instead of the private data for better privacy protection. Each client, the owner of private training data, updates a model locally, and sends all gradients or weights information to the cloud. The cloud aggregates such information from clients, updates a new central model (e.g., averaging all clients' weights), and then distributes it back to a fraction of clients for another round of model update. Such process is continued iteratively until a satisfying performance is achieved. Note that, to minimize communication, each client might take several mini-batch gradient descent steps in local model computation.
%\cite{mcmahan2016communication} first proposes the federated learning framework that can mitigate the privacy leakage of model training with limited, unbalanced, massively, or even non-IID data among distributed devices, such as mobile phones.
%In each round of communication between cloud and clients, the cloud aggregates all gradients or weights information from each client , updates a new central model (e.g., averaging all clients' weights), and then distributes it to a fraction of clients. 
%Next, the optimized models are sent back to the cloud and repeat the first step to update the central model.
%Depending on the performance of the central model, the training phase is stopped, or a new communication round starts. 
%However, the communication between cloud and clients might be limited and vulnerable to interception \cite{geyer2017differentially}.
To enhance the privacy protection, differential privacy has been applied to federated learning \cite{bhowmick2018protection,geyer2017differentially}. Previous works mostly focus on either the differential privacy mechanism that requires a central trusted party or the theoretical analysis of LDP techniques. Practical solutions for deep learning tasks data and tasks have not been well studied.



\section{Our Approach}


% In our setting, an aggregator collects data from a set of users and computes statistical models of the collected data. 
% Following the LDP model [2, 7, 11], we assume that the aggregator already knows the identities (e.g., IP addresses) of the
% users, but not their private data. Formally, let n be the
% total number of users, and ui (1 ≤ i ≤ n) denote the i-th
% user. Each user ui’s private data is represented by a tuple ti,
% which contains d attributes A1, A2, . . . , Ad. These attributes
% can be either numerical or categorical. Without loss of generality, we assume that each numeric attribute has a domain
% [−1, 1], and each categorical attribute with k distinct values
% has a discrete domain {1, 2, . . . , k}.
% To protect privacy, each user ui first perturbs her tuple ti
% using a randomized perturbation function f. Then, she sends
% the perturbed data f(ti) to the aggregator instead of her true
% data record ti. The perturbation function determines the
% privacy / utility tradeoff. As an extreme case, if f(ti) = ti
% (i.e., no perturbation), the aggregator obtains perfect utility
% since it computes the statistical models based on the exact
% data; however, the privacy of the users is completely lost
% as the aggregator receives their sensitive data. The other
% extreme is that f simply outputs a random tuple regardless
% of ti, which leads to the highest level of privacy and zero
% utility, i.e., the aggregator learns nothing about the users’
% data.

In the framework of \system\ as shown in Fig.\ref{fig:framework}, the cloud is an aggregator that collects a set of weights of local client models from the local side and averages the weights after each communication round. The goal is to maximize the accuracy of both cloud and local client models while preserving users' privacy. 
In our proposed algorithm, we will alter and approximate each local information with a randomized mechanism. This is done to totally hide a single client’s contribution within the aggregation and thus within the entire learning procedure.

\subsection{Threat Model}
Clients are honest-but-curious. They follow the training protocol and may try to infer information about other clients. In our design, clients do not share information with each other so they are unable to compromise each other's privacy. 

Cloud is not trusted. It may try to infer clients' private data based on model updates or weights collected from clients. It may utilize some auxiliary background knowledge to increase its inference capability.
We assume the majority of clients do not collude with the cloud.

%Our proposed framework aims to address the privacy challenges that arise in different clients by sharing deep learning models in federated learning setting. We assume that initially every client has the same initialization from the cloud and each local model then is trained using their own private data. We also assume that each client shares zero knowledge before privacy protection. All client also protect their privacy to the cloud side.
%In practice, we assume that the client will use their own dataset and training device, which requires the different training time locally. Various privacy and security risks arise in these scenarios, which we aim to address with our framework. In more detail, our threat model covers the following adversaries:

%\textbf{Malicious Cloud or Client} In federated learning, many parties try to get the private information by attacking or faking them as some participants. However, all privacy information are well-protected by the local differential privacy perturbation in our system since any communication is noisy information with theoretical guarantees.

Note that we do not intend to defend against active attacks such as data poisoning, which is a common problem in FL, but is out of the scope of this work.





\subsection{Overview of \system}

In this section, we introduce the federated learning approach with LDP consists of two steps, as shown in Algorithm \ref{alg:fedlocal}.

\noindent\textbf{Cloud Update.} 
First, the cloud initializes the weights randomly at the beginning.
Let $n$ be the total number of local clients.
Then, in the $r$-th communication round, the cloud will randomly select $k_r \leq n$ clients to update their weights for local-side optimization.
Unlike the previous works \cite{bhowmick2018protection,erlingsson2014rappor,seif2020wireless}, where they assume that the aggregator already knows the identities (e.g., IP addresses) of the users but not their private data, our approach assumes the client remains anonymous to the cloud. 

%We will show that this approach can provide us more robust privacy bound and practical solution.

%\noindent\textbf{Local Update.}
%For each client, it contains its own private dataset. In each communication, the selected local clients will update their local model by the weight from the cloud. Next, the local model uses Stochastic Gradient Descent (SGD) to optimize the distinct local models' weights in parallel. In order to provide a practical privacy protection approach, we split and shuffle each local model's weights and send each weight through an anonymous mechanism to the cloud. For splitting, we first separate all parameters of the trained model, and tag them with the location id. Then, we random generate a time $t$ in Algorithm \ref{alg:splitshuffling} to prevent the cloud to track the client owner of each parameter. For shuffling, we can use fake IP for each query from client to cloud, but there are also other practical solutions are well discussed in the split and shuffling section below. In this case, we can provide more reliable privacy protection and give a practical solution with available results in the final.

\noindent\textbf{Local Update.}
For each client, it contains its own private dataset.
In each communication, the selected local clients will update their local models by the weight from the cloud.
Next, each local model uses Stochastic Gradient Descent (SGD) \cite{RobbMonr51} to optimize the distinct local models' weights in parallel.
In order to provide a practical privacy protection approach,
each local client applies split and shuffle mechanism on the weights of local model and send each weight through an anonymous mechanism to the cloud.
For splitting, we separate all parameters of the trained model, and tag them with their location in the network structure.
For shuffling, we randomly generate a time $t$ in Algorithm \ref{alg:splitshuffling} to prevent the cloud to track the client owner of each parameter.
Detailed description and discussion on splitting and shuffling mechanism are given in the later section.


% In our proposed algorithm, we will alter and approximate each local information with a randomized mechanism. This is done to totally hide a single client’s contribution within the aggregation and thus within the entire decentralized learning procedure.

% \begin{algorithm}[t] 
% 	%\SetKwComment{tcp}{\tiny // }{}%
% 	\caption{{\system}
% 	} \label{alg:fedlocal}
%     \KwIn{$n$ is the number of local clients; $B$ is the local mini-batch size, $E$ the number of local epochs, $\gamma$ is the learning rate.}
% % 	\KwOut{}
% 	\tcp{Phase 1: Cloud Gradient Optimization}
% 	\textbf{CloudUpdate}\

%     Initialize weights $w_0$\;
% 	\For{each round $r = 1, 2, \ldots$ \label{line:cfor1}}{
% 		$k_r$ $\leftarrow$ random set of $f_r$ local clients, where $k_r \leq n$\;
% 		$\mathbf{W} \leftarrow clients(w_t, k_r)$; \% Collect all weights  from Clients\;
% 	    %}
% 	    \For{each $id \in \mathbf{W}$ \label{line:cfor2}}{
% 	    $w_{r+1}[id] \leftarrow \frac{1}{k_r} \sum_{(p,id,t) \in \mathbf{W}} p$; \% Take mean of each weight of local models by id and reformat $w_{r+1}$\;
% 	    }
% 	}
% 	$SendToClient(w_{t+1})$ \% Update clients\; 
% 	%\bf{return} $w_{t+1}$.
	
% 	\tcp{Phase 2: Local Gradient Optimization}
	
% 	\textbf{LocalUpdate($w, k_r$)}\
	
% 	Initialize weight information set $\mathbf{W}$\;
% 	\For{each local client $c \in k_r$ in parallel \label{line:cfor3}}{
% 	    $w_c \leftarrow w$\;
% 	    \For{each local Epoch $i = 1, 2, ...E$ \label{line:cfor4}}{
% 	        \For{each batch $b \in B$ \label{line:cfor5}}{
%                 $w_c \leftarrow w_c - \gamma \bigtriangledown L(w_c; b)$\;
%             }
%         }
%         $w_c^* \leftarrow DataPertubation(w_c)$\;
% 	    %$\mathbf{W} \leftarrow \mathbf{W} \cup {w_c^*}$ \;
% 	    $\mathbf{W} \leftarrow \mathbf{W} \cup SplittingShuffling(w_c^*)$\;
% 	}
% 	Order all $(p, id, t) \mathbf{W}$ by time $t$\;
% 	SendToCloud(p, id, t) based on time $t$\;
% 	%$\mathbf{W}^* \leftarrow $ Apply splitting and shuffling on $\mathbf{W}$\;
% 	% \bf{return} $\mathbf{W}^*$.
% \end{algorithm}

\subsection{Privacy-Preserving Mechanism} \label{sec:privacyprotection}


% \noindent \textbf{Differential Privacy}
% The second case is clients do not trust cloud and other clients, so they need to add DP locally, and the cloud will aggregate the noise gradient of each client. However, \textit{this is not LDP protection}, just apply differential privacy on local side, and we will discuss the difference later. 
% Then we can enforce a certain sensitivity by using scaled versions instead of the true updates: $\Delta \hat{w}^k = \Delta w^k / \max(1, \frac{\|\Delta w^k \|_2 }{S})$.
% Scaling ensures that the second norm is limited $\forall k, \|\Delta w^k \| < S$.
% The sensitivity of the scaled updates with respect to the summing operation is thus upper
% bounded by S.
% Different with last case, now each client adds noise (scaled to sensitivity S).
% Then, the cloud side to average client's output by $m_t$ yields an approximation,
% while preventing leakage of crucial information about an individual of each client.

% A new central model $w_{t+1}$ is allocated by adding this approximation to the current central model $w_t$.

% \[
%     \Delta \hat{w}^k = \underbrace{\overbrace{\Delta w^k / \max(1, \frac{\|\Delta w^k \|_2 }{S})}^{\text{An update clipped at S}} + \overbrace{\mathcal{N}(0,\delta^2 S^2)}^{\text{Noise scaled to S}}}_{\text{Gaussian mechanism approximating sum of update}}
% \]

% \[
%     w_{t+1} = w_t + \frac{1}{m} \underbrace{\sum_{k=0}^{m_t}\Delta \hat{w}^k}_{\text{Sum of updates clipped at S}}
% \]

\noindent \textbf{Data Perturbation.}
Given the weights $W$ of a model, the algorithm returns a perturbed tuple $W^*$
by randomizing each dimension of $W$. Let $\cM$ be our mechanism, for each weight/entry $w\in W$, assuming $w\in [c-r, c+r]$ where $c$ is the center of $w$'s range and $r$ is the radius of the range ($c,r$ depend on how we clip the weight).
As an alternative notation, if $w\in[a,b]$, then $c=(a+b)/2, r=(b-a)/2$.
We generalize the LDP mechanism in~\cite{duchi2018minimax} so the input can be in any interval. We perturb $w$ to $w^*$ with two intuitions.
First, $w^*$ can only be one of two discrete values: one larger, the other smaller, which makes it easy to prove LDP. Then, to ensure the noise has zero mean, i.e., $\mathbb{E}(w^*)=w$, we set $w^*$ to the larger value with a high probability if $w$ itself is large, and set $w^*$ to the smaller value with a high probability if $w$ itself is small.
Therefore, we design the following LDP mechanism to perturb $w$.

\begin{equation}
\begin{aligned}
\label{eq:ldp}
    w^* &=\cM(w) \\
    &= 
\begin{cases}
    c + r\cdot \frac{e^\epsilon+1}{e^\epsilon-1}, \text{   w.p.   }\frac{(w-c)(e^\epsilon - 1)+r(e^\epsilon+1)}{2r(e^\epsilon+1)}\\ \\
    c - r\cdot \frac{e^\epsilon+1}{e^\epsilon-1},  \text{   w.p.   }\frac{-(w-c)(e^\epsilon - 1)+r(e^\epsilon+1)}{2r(e^\epsilon+1)}
\end{cases}
\end{aligned}
\end{equation}
where $w^*$ is the reported noisy weight by our proposed LDP, and ``w.p.'' stands for the ``with probability''. 
Algorithm \ref{alg:noise} shows the pseudo-code of this mechanism. 

%\vspace{10px}
%\begin{minipage}{0.46\textwidth}
\begin{algorithm}[t]
    \caption{{\system}
	} \label{alg:fedlocal}
    \KwIn{$n$ is the number of local clients; $B$ is the local mini-batch size, $E$ the number of local epochs, $\gamma$ is the learning rate.}
% 	\KwOut{}
	%\tcp{Phase 1: Cloud Gradient Optimization}
	\textbf{CloudUpdate}\

    Initialize weights $W_0=\{w^0_{id}\mid \forall id\}$, where $id$ indicates the position of each weight\;
    $SendToClient(W_{0})$\;
	\For{each round $r = 1, 2, \ldots$ \label{line:cfor1}}{
		randomly select $k_r (k_r \leq n)$ local clients\;
		collect all weights $\cW = \{(id, w_{id}, t)\mid \forall id, t\}$ from selected clients with $SendToCloud$ \;
	    %}
	    \For{each $id \in \cW$ \label{line:cfor2}}{
	    $W_{r}[id] \leftarrow \frac{1}{k_r} \sum_{id, w,t) \in \cW} w$; \% Compute mean of each weight of local models by id\;
	    }
	    $SendToClient(W_{r}, k_r)$ \% Update clients\; 
	}
	%\bf{return} $w_{t+1}$.
	
	%\tcp{Phase 2: Local Gradient Optimization}
	
	\textbf{LocalUpdate($W_r, k_r$)}\
	
	Receive weights $W_r$ from cloud by $SendToClient$\;
	\For{each local client $c \in k_r$ in parallel \label{line:cfor3}}{
	    $W^c_r \leftarrow W_r$\;
	    \For{each local epoch $i = 1, 2, ...E$ \label{line:cfor4}}{
	        \For{each batch $b \in B$ \label{line:cfor5}}{
                $W^r_c \leftarrow W^r_c - \gamma \bigtriangledown L(W^r_c; b)$\;
            }
        }
        ${W^r_c}^* \leftarrow DataPertubation(W^r_c)$\;
	    %$\mathbf{W} \leftarrow \mathbf{W} \cup {w_c^*}$ \;
	    ${\cW^r_c}^* \leftarrow SplitShuffle({W^r_c}^*)$\;
%	    \tcp{Send the pair information back to cloud by time $t$}
	    $SendToCloud(id, w, t)$ by ascending time $t$, $ \forall (id, w, t) \in {\cW^r_c}^*$\;
	}
	%$\mathbf{W}^* \leftarrow $ Apply splitting and shuffling on $\mathbf{W}$\;
	% \bf{return} $\mathbf{W}^*$.
\end{algorithm}
%\end{minipage}
%\hfill
%\begin{minipage}{0.46\textwidth}
\begin{algorithm}[] 
    \caption{DataPertubation	
	} \label{alg:noise}
	\KwIn{Original $W$.}
	\KwOut{$W^*$ after data perturbation}
    Prefix the range of the $W$ and then we have fixed $c$ and $r$\;
	
	\For{each weight $w \in W$ \label{line:cfor6}}{
		Sample a Bernoulli variable $u$ such that\\
		$\Pr[u=1]=  \frac{(w-c)(e^\epsilon - 1)+r(e^\epsilon+1)}{2r(e^\epsilon+1)}$\;
		\If{u==1}{
		    $w^* = c + r\cdot \frac{e^\epsilon+1}{e^\epsilon-1}$\;
		}
		\Else{
		    $w^* = c - r\cdot \frac{e^\epsilon+1}{e^\epsilon-1}$\;
		}
		replace $w$ with $w*$\;
	}
	After perturb all $w \in W$, we have $W \rightarrow W^*$\;
	\bf{return} $W^*$.
\end{algorithm}
%\vspace{15px}
\begin{algorithm}[t]
    \caption{SplitShuffle	
	} \label{alg:splitshuffling}
	\KwIn{Perturbed $W$ after Algorithm \ref{alg:noise}}
	\KwOut{$\cW^*$ after shuffling approach}
    	Initialize a weight information set $W^*$\;
	\For{each weight $w \in W$ and its position id $id$ \label{line:cfor7}}{
	    $t \leftarrow$ Randomly sample a small latency $t$\;
	    $\cW^* \leftarrow \cW^* \cup (id, w, t)$\;
	}
	\bf{return} $\cW^*$.
\end{algorithm}
%\end{minipage}
%\vspace{10px}

%=====================================================
\begin{figure*}[tb]
\centering
\includegraphics[width=5.5in]{figures/NIPS20-shuffling1.pdf}
\caption{Example of splitting and shuffling in \system. Note that, the splitting and shuffling is done locally instead of by a third party. This figure demonstrates that after the splitting and shuffling mechanism, the cloud will aggregate what kind of information from clients.} \label{fig:shuffling}
\end{figure*}
%======================================================

In previous mechanisms \cite{abadi2016deep,papernot2017semi}, the generated noisy data is close to its original value with high probability, still revealing information, whereas our approach makes the noisy data very distinct from its original value.
For example, while $c=0, r=1$ and $\epsilon=1$, the perturbed information only could be either $\frac{e+1}{e-1} \approx 2.163953$ or $ -1.0 \cdot \frac{e+1}{e-1} \approx -2.163953$ for any the original data.

\noindent \textbf{Adaptive Range Setting.}
For any weight $w \in [c - r, c + r]$, previous approaches \cite{xxx} have prior knowledge to set the fixed range of the task. However, it brings a coming questions: How to get the prior knowledge, especially for a complex deep learning method? In fact, prior knowledge is a very strong assumption and all clients having a consensus at the beginning is not very practical in most scenarios .
Assuming there is no prior knowledge for all clients, a naive solution is to set a very large range which can probability cover all clients.
However, due to the larger variance of the expectation of the noisy mean of the clients' weights, the utility would be bad, especially for deep learning due to its complex structure and different range of the weights in each layer.

In order to tackle this issue, we propose adaptive range setting during the federated learning.
For each step, besides to send the perturbed weight to the server,
each client also sends the encrypted min- max pair value of each layer in anonymity to the server.
Though a encrypted min-max computation, the server will return the encrypted min-max value to the client though all clients.
Last, the clients can decrypt the min-max value and use them to set up the range of the values for LDP perturbation.


% \begin{algorithm}[t] 
% 	\caption{DataPertubation(w)	
% 	} \label{alg:noise}
% % 	\KwIn{Graph $G=(V,E,w)$, Seed Set $S$, budget $q$, accuracy weights $(\epsilon, \ell)$}
% % 	\KwOut{Edge $F$}
% 	
%     Prefix the range of the $w$ and then we have fixed $c$ and $r$\;
% 	
% 	\For{each weight $p \in w$ \label{line:cfor6}}{
% 		Sample a Bernoulli variable $u$ such that\\
% 		$\Pr[u=1]=  \frac{(p-c)(e^\epsilon - 1)+r(e^\epsilon+1)}{2r(e^\epsilon+1)}$\;
% 		\If{u==1}{
% 		    $p^* = c + r\cdot \frac{e^\epsilon+1}{e^\epsilon-1}$\;
% 		}
% 		\Else{
% 		    $p^* = c - r\cdot \frac{e^\epsilon+1}{e^\epsilon-1}$\;
% 		}
% 		replace $p$ as $p*$\;
% 	}
% 	After perturb all $p \in w$, then we have $w \rightarrow w^*$\;
% 	\bf{return} $w^*$.
% \end{algorithm}
% 
% \begin{algorithm}[t] 
% 	%\SetKwComment{tcp}{\tiny // }{}%
% 	\caption{SplittingShuffling(w)	
% 	} \label{alg:splitshuffling}
% 	
% 	Initialize a weight information set $w^*$\;
% 	\For{each weight and its id $(p, id) \in w$ \label{line:cfor7}}{
% 	    $t \leftarrow$ Random Sample a Time\;
% 	    $w^* \leftarrow w^* \cup (p, id, t)$\;
% 	}
% 	\bf{return} $w^*$.
% \end{algorithm}

\noindent \textbf{Splitting \& Shuffling.}
As pointed in \cite{dwork2014algorithmic}, a sophisticated privacy-preserving system composites multiple locally differentiate algorithms leads to a composition of privacy cost of such algorithms. That is, a combination of locally differentiate algorithm with privacy budget $\epsilon_1$ and $\epsilon_2$ consumes a privacy budget of $\epsilon_1 +\epsilon_2$. Training a deep neural network using federated learning requires clients to upload gradient update to the cloud in multiple iterations. If location differential privacy is applied at each iteration, along the iterative training process, the privacy budget will accumulate and case the explosion of the total privacy budget. In order to control the total privacy budget, a larger noise has to be added in the algorithm which inevitably hurts the model's accuracy for complex learning task.

Bittau et al. designed the \textit{Encode, Shuffle, Analyze} (ESA) architecture which leverages trustworthy shufflers to anonyomize LDP reports from users in order to enhance privacy protection. This idea was further formalized by Erlingsson et al. \cite{erlingsson2019amplification}. It is shown that when LDP reports are properly anonymized at each timestep and unlinkable over the time, the overall privacy guarantee can be greatly improved. Inspired by their work, we proposed to add anonymity into the proposed protocol so that the cloud is unable to \textit{directly} link the received data with a specific client, for the benefits of better privacy protection. Such anonymization can be achieved by multiple existing mechanisms, depending on how the server tracks clients in the specific scenario. As a typically best practice for privacy, a certain level of anonymity of each client to the server is applied to disassociate clients' individually-identifiable information from their weights update. For example, if the server tracks clients by IP address, each client can adopt an untraceable IP address by using a network proxy, a VPN service \cite{OperaVPN}, a public WiFi access, and/or the Tor \cite{Dingledine04tor}. For another example, if the server tracks clients by a software-generated metadata such as an ID,  each client can randomize this metadata before sending it to the server. More advanced anonymization techniques have also been proposed such as using secure multiparty computation \cite{Bonawitz2017}.


%Due to the high data dimension and multi round interaction between cloud %and clients for model training, the traditional approach will cause the %explosion of the privacy cost.
%To tackle the issues, 
%we assume the clients utilize existing anonymization techniques to disassociate their personally-identifiable information from their uploaded data. client anonymity can be achieved via faking source IP, VPN, proxy, Tor, secure multi-party computation, etc~\cite{erlingsson2019amplification}, which is a typical approach to enhance privacy.
However, we argue that client anonymity is not sufficient to prevent side-channel linkage attack, e.g., the cloud can still link a large number of data together if the client uploaded them at the same time.
Therefore, we design the local splitting and shuffling mechanism break the updates into pieces.
The primary purpose is to give stronger privacy protection while using LDP on federated learning. Compared to traditional machine learning, deep learning needs more communications and weights for better performance, causing more privacy leakage during traditional federated learning. So, splitting and shuffling can greatly reduce privacy budget during the training phase.

% First, \system\ will split gradients or weights after local training and sending each gradient/weight with different dummy IP addresses.
% Each IP address only collects the weight in the original order of the model structure from each local client.  
% Then, before sending the weights to the cloud, each client needs to shuffle the order of all weights in each IP address.
% After splitting and shuffling, the cloud can not link the weights and the client back, so it can reduce the information leak for the user.
% Alternatively, we can also ask all clients to use the same dummy IP so that it looks like all data are from the same client from the cloud's perspective.
Splitting breaks the private connections of each local client model's weights, and shuffling mixes all clients' weights together and makes them indistinguishable from each other. An approach is given in Algorithm~\ref{alg:splitshuffling}, where each client samples a small random latency $t$ for each weight and waits $t$ before sending the weight to the cloud.
Fig.~\ref{fig:shuffling} shows the idea of splitting and shuffling of the weights of each local client model that contains two main steps. For local model $A, B, C$, each model has the same structure but with different weight values. Original federated learning is to send the models' information to the cloud, as shown in Fig.~\ref{fig:shuffling} (1). In our approach, first, for each model, we split the weights of each local model. Then, for each client, we shuffle the weights though random latency and send each weight with its id to the cloud, where id indicates the location of the weight value in the network structure. Finally, splitting and shuffling can ensure the cloud collects the right weight values to update the central model without any knowledge about the relation of each weight and local clients.
Note that \system\ supports each client to finish the split and shuffling locally instead of using a third party.

% In practise, each client fakes their IP address as a new IP address in each communication (same as shuffling).
% Meanwhile, each client splits their weights and send them separately to the cloud (same as splitting). Note that, the client will tell a message, which contains which weight of the model.
% Through above approach, the cloud does not know the received information from which local client.
% In this case, cloud can never recover the original weights from a particular client in any communication. The privacy can be better protected.

%In practice, client anonymity can be achieved via faking source IP, VPN, proxy, Tor, secure multi-party computation, etc~\cite{erlingsson2019amplification}. How to achieve anonymity is not the focus of our work.
Splitting and shuffling breaks the linkage between model updates from the same clients and hides them among updates from other clients, making it harder for the cloud to combine more than one piece of updates to infer more information about any client.
Note that the shuffling in~\cite{erlingsson2019amplification} is achieved by a semi-trusted third-party, for the purpose of achieving centralized DP on the cloud providing statistics for an untrusted analyst. On the contrary, our shuffling is performed locally to strength local DP.




%\subsection{Client Anonymity}
%Additionally, as a typically best practice for privacy, a certain level %of anonymity of each client to the server is applied to disassociate %clients' individually-identifiable information from their weights %update, so that the cloud is unable to \textit{directly} link the %received data with a specific client. Such anonymization can be achieved %by multiple existing mechanisms, depending on how the server tracks %clients in the specific scenario. For example, if the server tracks %clients by IP address, each client can adopt an untraceable IP address %by using a network proxy, a VPN service \cite{OperaVPN}, a public WiFi %access, and/or the Tor \cite{Dingledine04tor}. For another example, if %the server tracks clients by a software-generated metadata such as an %ID,  each client can randomize this metadata before sending it to the %server.

% the cloud can random assign a new IP address in each communication.
% Then, all client sends the protected results to the new IP address. Next, the new IP address can random shuffling the order of weights by client.
% Finally, the new IP address send all protected weights with random order to the cloud.
% After cloud update the new central model, the cloud will repeat the first step to reassign a new IP address. In this case, cloud can never recover the original weights from a particular client in any communication. The privacy can be better protected.

\section{Privacy and Utility Analysis} \label{sec:privacy}
In this section, we analyze the privacy guarantee and utility cost of our approach, and compare it with other LDP mechanisms. Due to limited space, all proofs of lemmas and theorems are given in the appendix.

\subsection{Local Differential Privacy}
We prove the proposed random noise addition mechanism $\cM$ satisfies LDP.

\begin{restatable}{theorem}{epsproof}
Given any single number $w \in [c-r, c+r]$, where $c$ is the center of $w$'s range and $r$ is the radius of the range, the proposed mechanism $\cM$ in Eq.~\ref{eq:ldp} satisfies $\epsilon$-LDP.
\end{restatable}

% \begin{proof}
% We know the weight $p$'s range is $[c-r, c+r]$.
% If $p^*=c+r\cdot\frac{e^\epsilon+1}{e^\epsilon-1}$, then for any $p,p'\in[c-r, c+r]$.
% \begin{equation}
% \dfrac{\Pr[\mathcal{M}(p)=p^*]}{\Pr[\mathcal{M}(p')=p^*]}\le \dfrac{\underset{p}{\max}\Pr[\mathcal{M}(p)=p^*]}{\underset{p'}{\min}\Pr[\mathcal{M}(p')=p^*]} = \dfrac{r(e^\epsilon-1)+r(e^\epsilon+1)}{-r(e^\epsilon-1)+r(e^\epsilon+1)} = e^\epsilon.
% \end{equation}
% If $p^*=c-r\cdot\frac{e^\epsilon+1}{e^\epsilon-1}$, the above still holds.
% \end{proof}

%we actually transmit all weights of each local client to the same IP address.
%In Algorithm \ref{alg:noise}, unlike previous works，we observe that in the above method, the output $w^∗_i$ contains $\theta$ non-zero value, for the randomly chosen attribute $A_j$, where $\theta = |w^*_i|$.  % our mechanism doesn't select dimension, so no need to mention this.
%It makes all weights of a single user is individual to each other, hence, the user $u_i$ only needs to transmit 1 bit for each private weight to the cloud aggregator indicating its sign.  %irrelavant to us
%Further, as we show below the correctness of this method does not depend on the choice of $A_j$ as long as it is chosen uniformly at random. Therefore, the value of j can be obtained, e.g., using a public source of random numbers such as a hash value of the user’s ID. Therefore, the communication overhead between each user and the aggregator is exactly 1 bit. %irrelavant to us

%The following lemmas establish the theoretical guarantees of Algorithm \ref{alg:noise}.

\subsection{Splitting and Shuffling}
As we claimed before, \system\ uses splitting and shuffling to bypass the curse of dimensionality.
Since the weights are split and uploaded anonymously, the cloud is unable to link different weight values from the same client, so it cannot infer more information about a particular client. Therefore, it is sufficient to protect $\epsilon$-LDP for each weight. Likewise, because of the client anonymity, the cloud is unable to link weights from the same client at different iterations.
Without splitting and shuffling, the privacy budget of LDP will grow to $Td\epsilon$, where $T$ is the iteration number and $d$ is the number of weights in the model.
Similar discussion can be found in~\cite{erlingsson2014rappor,erlingsson2019amplification}. Unlike our approach, the previous works shuffle the ordered sequential information.

\subsection{Bias and Variance}
Suppose the true average weights in an iteration is $\Bar{w}=\dfrac{1}{n}\sum_u w_u$ for each $w \in W$, the proposed LDP mechanism in Eq.~\ref{eq:ldp} induces zero bias in calculating the average weight $\overline{\mathcal{M}(w)}=\dfrac{1}{n}\sum_u \mathcal{M}(w_u)$.
\begin{restatable}{lemma}{noiseproof}
\label{th:bias}
Algorithm~\ref{alg:noise} introduces zero bias to estimating average weights, i.e., $\mathbb{E}[\overline{\mathcal{M}(w)}]=\Bar{w}$.
\end{restatable}
%Lemma~\ref{th:bias} shows that if we have infinite number of clients, the cloud can get an zero-bias central model by averaging the perturbed weights.
Lemma~\ref{th:bias} indicates that if we have more client, the average of the perturbed weights is closer to the true average.

The following lemmas show the variance of the data obtained by the cloud.
First, the proposed mechanism leads to a variance to each reported weight $\mathcal{M}(w)$. 
\begin{restatable}{lemma}{varcmpproof}
\label{lemma:cmp}
Let $\cM$ be the proposed data perturbation mechanism. Given any number $w$, the variance of the mechanism is
$Var[\mathcal{M}(w)] =r^2O(e^{-\epsilon}+e^{-2\epsilon}).$
\end{restatable}
Then, for the variance of the estimated average weight $\overline{\mathcal{M}(w)}$,
we have the lower bound and upper bound as below.
\begin{restatable}{lemma}{varianceproof}
\label{lemma:var}
Let $\overline{\mathcal{M}(w)}$ be the estimated average weight. The lower bound and upper bound of the estimated average weight is:
$\dfrac{r^2(e^\epsilon+1)^2}{n(e^\epsilon-1)^2}-\dfrac{r^2}{n} \le Var[\overline{\mathcal{M}(w)}] \le \dfrac{r^2(e^\epsilon+1)^2}{n(e^\epsilon-1)^2}.$
\end{restatable}
It can be seen from Lemma \ref{lemma:var} that, with enough clients (a large $n$), we can achieve a low variance on the estimated average weight with a wide range of perturbed data (a large $r$) and a small privacy cost (a small $\epsilon$). 
%The variance is large when $r$ is large, $\epsilon$ is small, or $n$ is small.
With the above lemmas, we conclude the following theorem that shows the accuracy guarantee for calculating average weights on the cloud.
\begin{restatable}{theorem}{boundproof}
For any weight $w\in W$, with at least $1-\beta$ probability,
\begin{equation*}
|\overline{\mathcal{M}(w)}-\Bar{w}|<O\left(\dfrac{r\sqrt{-\log\beta}}{\epsilon\sqrt{n}}\right).
\end{equation*}
\end{restatable}


% The previous two lemmas
% The variance and the upper/lower bound analysis show the proposed mechanism can well support the aggregator to achieve a closer average to the true average on the perturbed information while increasing the number of the clients $n$. We also compared the proposed mechanism to other existing mechanisms, and find an interesting discovery. More details are shown and discussed in the next two sections.
% Then, the following corollary states the accuracy guarantee of our solution for weight $p \in w$ of any local model.
\iffalse
\subsection{Comparison with Other Mechanisms}
First, existing mechanisms generate noisy data that is close to its original value w.h.p., revealing the original value's confidence interval. For instance, Laplace and Gaussian mechanisms add small noise w.h.p. and randomized response based mechanisms keep the data unchanged w.h.p. 
On the contrary, the proposed mechanism chooses one out of two extreme values as the noisy data, making it more distinct from its original value. 
Then, we compare with the following popular mechanisms specifically. 

\textit{Randomized Response Mechanism.}
Google's Rappor~\cite{erlingsson2014rappor} and generalized randomized response~\cite{wang2017locally} are for binary or categorical data only, whereas data are numeric in the scenario of federated learning.

\textit{ScalarDP~\cite{bhowmick2018protection}.}
%ScalarDP introduces a variance $r_{max}^2O(-2\epsilon/3)$ to the noisy data (Lemma 4.4 in~\cite{bhowmick2018protection}), whereas our variance bound is tighter (Lemma~\ref{lemma:cmp}). Besides, t
This work~\cite{bhowmick2018protection} assumes the attacker has little prior knowledge about user data and that $\epsilon$ is very large.

\textit{Laplace Mechanism~\cite{dwork2014algorithmic}.}
If we apply the Laplace mechanism to each client's data $w$, the variance is $\text{Var}[\mathcal{M}(w)] =2\frac{\Delta^2}{\epsilon^2}=\frac{8r^2}{\epsilon^2}$.
The variance of estimated average over $n$ clients is $\text{Var}[\overline{\mathcal{M}(w)}]=\frac{\text{Var}[\mathcal{M}(w)]}{n}=\frac{8r^2}{n\epsilon^2}$.
%, which is higher than ours (Equation~\ref{eq:var}) when $\epsilon<2.3$ at least. 
In our best case (Equation~\ref{eq:var}), the Laplace mechanism's variance is always higher than ours for any $\epsilon$.
We also compare with Laplace in terms of absolute data perturbation $|w^*-w|$ to prove our mechanism is securer in the appendix. For instance, when $\epsilon=1$, our data perturbation is greater than Laplace's with probability 0.79 in the best case. Therefore, we claim our mechanism makes noisy data more distinct from its original value than Laplace mechanism.
%The advantages of the Laplace mechanism include that it is easier to understand, and the noisy data is still continuously distributed.

\textit{Gaussian Mechanism~\cite{dwork2014algorithmic}.}
Currently, most works on $\epsilon$-LDP do not relax its definition with $\delta$.
However, the Gaussian mechanism introduces $\delta$ \cite{dwork2014algorithmic}, making it weaker than LDP \cite{duchi2014privacy}. 
$\delta$ is the probability that indicates those highly unlikely ``bad'' events. 
These ``bad'' events may break $\epsilon$-differential privacy and usually defined by the size of the dataset in previous works \cite{papernot2017semi,wang2018private}.
As a result, the Gaussian Mechanism is less secure than our mechanism (without introducing $\delta$).
\fi

% \subsection{Discussion: DP vs LDP}
% There is a blurry line between DP and LDP. In general, they differ in definition and in whether the noise is added locally or on the server. However, they are not mutually exclusive. The definition of LDP is a special case of that of DP. Also, sometimes noises are added locally to achieve DP instead of LDP, e.g., via additive secret sharing.

% We can prove that any mechanism for DP can also be used to achieve LDP. 
% \begin{restatable}{thm}{dptoldpproof}
% Let $\cM$ be any mechanism satisfying $\epsilon$-differential privacy. Applying $\cM$ to each value of a dataset containing $k$ values satisfies $k\epsilon$-LDP.
% \end{restatable}



\section{Experiments}

%=====================================================
\begin{figure}[t]
\centering
\subfloat[Communication Round]{\includegraphics[width=1.7in]{figures/diff_epoch_1 .png}}
\subfloat[Fraction of Clients]{\includegraphics[width=1.7in]{figures/diff_frac_1.png}}
\caption{Parameter analysis on communication round and fraction of clients. For MNIST, Fashion-MNIST and CIFAR-10, we set the number of total clients as 100, 200, 500 respectively.} \label{fig:param}
\end{figure}
%======================================================

%=====================================================
\begin{figure*}[tb]
\centering
\subfloat[Effect of $n$ on MNIST ($\epsilon=1$)]{\includegraphics[width=1.73in]{figures/mnist_usernum.pdf}}\ \ \
\subfloat[Effect of $n$ on Fashion-MNIST ($\epsilon=5$)]{\includegraphics[width=1.73in]{figures/fmnist_usernum.pdf}}\ \ \
\subfloat[Effect of $n$ on CIFAR ($\epsilon=10$)]{\includegraphics[width=1.73in]{figures/cifar_usernum.pdf}}\\
\subfloat[Effect of $\epsilon$ on MNIST ($n=100$)]{\includegraphics[width=1.73in]{figures/mnist_eps.pdf}} \ \ \
\subfloat[Effect of $\epsilon$ on Fashion-MNIST ($n=200$)]{\includegraphics[width=1.73in]{figures/fmnist_eps.pdf}} \ \ \
\subfloat[Effect of $\epsilon$ on CIFAR ($n=500$)]{\includegraphics[width=1.73in]{figures/cifar_eps.pdf}} \\
\caption{Effect of $n$ and $\epsilon$ on the training accuracy .} \label{fig:budget}
\end{figure*}
%======================================================

\begin{table*}[tb]
    \centering
  \caption{Summary of Accuracy and Privacy Budget Analysis} \label{table:performance}
  %\resizebox{3.350in}{!}{%
  \begin{tabular}{|l|c|c|c|c|c|c|}
\hline
                   & noise-free   & $\epsilon$=0.1 & $\epsilon$=0.5 & $\epsilon$=1   & $\epsilon$=5   & $\epsilon$=10  \\ \hline
%MNIST (n=100)      & 97.26\% & -       & -       & -       & -       & -       \\ \hline
MNIST-LDP  (n=100) & 97.26\% & 13.84\% & 95.36\% & 96.24\% & 96.34\%       & 96.39\%       \\ \hline
%Fashion-MNIST (n=200)      & 87.53\% & -       & -       & -       & -       & -       \\ \hline
Fashion-MNIST-LDP  (n=200) & 87.53\% & 10.00\% & 10.00\% & 68.21\% &    85.95\%    & 86.10\%       \\ \hline
%CIFAR (n=500)      & 61.46\% & -       & -       & -       & -       & -       \\ \hline
CIFAR-LDP (n=500)  & 61.46\% & 10.00\%       & 10.00\%       & 10.00\% & 58.89\% & 60.37\% \\ \hline
\end{tabular}
  %}
\end{table*}

In this section, image classification tasks and a real mobile application are used as experimental examples to evaluate the effectiveness of \system. We first examine the effect of different weights based on the image benchmark datasets, MNIST \cite{LeCun1998}, Fashion-MNIST \cite{xiao2017fashion} and then verify the performance improvement based on CIFAR-10 \cite{krizhevsky2009learning} and the preceding three datasets. 

% For image classification tasks, three widely used convolutional deep neural networks (Conv-Small, VGG-Small) are implemented in \system\ \cite{Laine2017, Park2017}.
% For MNIST, we use Conv-Small as the cloud-side DNN. In the performance comparison, VGG-Small is used for CIFAR-10.
% To verify the performance improvement brought by \system, we need to mainly evaluate the performance with the number of the client.
For MNIST and Fashion-MNIST, we implement a two-layer CNN for image classification. However, for CIFAR-10, the default network from Pytorch library only achieves around 50\% accuracy without data perturbation, and we re-design a small VGG \cite{simonyan2014very} for the task.
The training data and the testing data are fed into the network directly in each client, and for each client, the size of the training data is the total number of the training samples divides the number of the clients.
In this case, a larger number of clients implicits the small size of the training data of each client.
For each weight, we clip them in a fixed range. In this work, we set $(c, r)=(0, 0.075)$ and $(0, 0.015)$ for MNIST and Fashion-MNIST, respectively. For CIFAR-10, due to the complexity of the network, we set $c=0$ and $r$ is adaptively set by the weight range of each layer, using the max value minus min value of each layer.
The learning rate $\gamma$ is set as 0.03 for MNIST/Fashion-MNIST and 0.015 for CIFAR-10.
Considering the randomness during perturbation, we run the test experiments ten times independently to obtain an averaged value.
In order to evaluate the performance of different learning approaches, we use different metrics including accuracy for utility, $\epsilon$ for privacy cost and $n$ communication rounds for communication cost. Any approach with a high accuracy, a small $\epsilon$ and a small communication round indicates a good and practical solution.

The proposed models are implemented using Pytorch, and all experiments are done with a single GPU NVIDIA Tesla V100 on the local server. 
MNSIT and Fashion-MNIST can be within an hour with 10 communication rounds, and CIFAR-10 needs about 2 hours with 15 communication rounds.



\subsection{Parameter Analysis}


In order to evaluate the performance of the \system, we need to fine-tune different parameters in the system.
Here we discuss two most critical parameters, i.e., the total number of communication rounds $R$, and the fraction of clients selected to update the global model in each communication $f_r = k_r / n$, where $k_r$ is the number of selected clients in round $r$, 
%$r$ is the number of current communication round, $r \in R$
and $n$ is the total number of clients, respectively.
%The fraction of clients $f_r$ denotes the random select the percentage of the clients to update the global model in each communication.

Fig.~\ref{fig:param} shows the change of the performance with varying $f_r$ and $R$. In this work, we evaluate the proposed model on MNIST, Fashion-MNIST and CIFAR.
To evaluate the parameter $f_r$, we first fix the number of the client as 500. It can be found that when $f_r$ is too small, it does not affect the performance on MNIST, but affects significantly the performance on Fashion-MNIST and CIFAR-10.
When $f_r$ is close to 1, \system\ can achieve almost the same performance as the noise-free results on MNIST, Fashion-MNIST and CIFAR-10, as shown in Table \ref{table:performance}.
Another important parameter is the communication rounds between cloud and clients. It is not hard to see that with more communications, we can train a better model on MNIST, Fashion-MNIST and CIFAR-10 through the proposed model. However, due to the complexity of data and tasks, CIFAR-10 needs more communication rounds for a better model.

%The federated learning approach is an open-source \footnote{The open source implementation given in \url{https://github.com/AshwinRJ/Federated-Learning-PyTorch}}, and our code will be released soon.

% The proposed models are implemented using Pytorch \cite{Tensorflow}. For image classification tasks, the learning rate and batch size are set as 0.03 and 10, respectively. The numbers of epochs for MNIST, and CIFAR-10 are 10 and 100, respectively. Considering the randomness during perturbation, we run the test experiments ten times independently to obtain an averaged value. The code is provided for reproducibility.




% %=====================================================
% \begin{figure*}[tb]
% \centering
% \subfloat[MNIST (5,10\%)]{\includegraphics[width=1.625in]{figures/mnist-p.jpg}}\ \ \
% \subfloat[SVHN (2,5\%)]{\includegraphics[width=1.625in]{figures/svhn-p.jpg}}
% \caption{Effect of $\eta$ and $\lambda$.} \label{fig:parameter}
% \end{figure*}
% %======================================================




\subsection{Performance Analysis and Comparison}


Fig. \ref{fig:budget} shows that \system\ can achieve a high accuracy with a low privacy cost because of the new design of the communication and the new local data perturbation. While increasing the number of clients $n$ in training, the \system\ can perform as close as the noise-free federated learning. Compared with MNIST ($n=100$), Fashion-MNIST ($n=200$), CIFAR-10 ($n=500$) needs more clients, which indicates that for a more complex task with a larger neural network model, it requires more local data and more clients for a better performance against the data perturbation. The privacy budget also affects the performance of the central model, but more details will be discussed in the next section.

\textbf{Compared with other baselines}
\system\ can achieve 96.24\% accuracy with $\epsilon=1$ and $n=100$, 86.26\% accuracy with $\epsilon=4, n=200$ and 61.46\% accuracy with $\epsilon=10, n=500$ on MNIST, Fashion-MNIST and CIFAR-10, respectively. 
Our results are very competitive comparing to other previous works.
Geyer et al. \cite{geyer2017differentially} first apply DP on federated learning. While they use $100$ clients, they can only achieve 78\%, 92\% and 96\% accuracy with $(\epsilon, n) = (8, 11)$, $(8, 54)$ and $(8, 412)$ guaranteed on MNIST with central differential privacy, where $(\epsilon, n)$ represents the privacy budget and the communication rounds.
Bhowmick et al.\cite{bhowmick2018protection} first utilize the LDP in federated learning. Due to the high variance of their mechanism,  it requires more than 200 communication rounds and spends much more privacy budgets, \textit{i.e.,} MNIST ($\epsilon=500$) and CIFAR-10 ($\epsilon=5000$). 
Last, the most recent work \cite{truex2020ldp} utilizes Condensed Local Differential Privacy ($\alpha$-CLDP) into federated learning, with 86.93\% accuracy on Fashion-MNIST dataset. However, $\alpha$-CLDP achieved that performance by requiring a relatively privacy budget $\epsilon = \alpha \cdot 2c \cdot10^\rho$ (e.g. $\alpha=1, c=1, \rho=10$), which results in a weak privacy guarantee. Compared to existing works, our approach can first use much fewer communication rounds between clients and cloud (\textit{i.e.,} 10 for MNIST, 15 for Fashion-MNIST and CIFAR-10), which makes the whole solution more practical in real scenarios.
Overall, \system\ achieves better performance on both effectiveness and efficiency than relevant works.
% Note that we only focus on federated learning with privacy protection in this paper, comparison with other communication approaches with privacy protection that does not apply to federated learning, such as PATE \cite{papernot2017semi,papernot2018scalable}, is out of scope.


\subsection{Analysis of Privacy Budget}

%The privacy budget represents the privacy cost in the framework. 
To analyze the impact of privacy budgets on performance, we present the accuracy results with privacy budget from 0.1 to 1 for MNIST, 1 to 10 Fashion-MNIST and 1 to 10 for CIFAR-10 in Figure \ref{fig:budget} (d-f).
It shows that \system\ can maintain the accuracy at a high value for a wide range of privacy budgets on MNIST ($\epsilon > 0.3$), Fashion-MNIST ($\epsilon > 2$) and CIFAR-10 ($\epsilon > 5$).
While $\epsilon<0.3$ for MNIST and $\epsilon < 5$, the accuracy decreases by 90\% ($\epsilon=0.1$), 15\% ($\epsilon=1$) and 50\% ($\epsilon=1$) for MNIST, Fashion-MNIST and CIFAR-10, respectively.
It is obvious that more complex data and tasks require more privacy cost.
The main reason is that the complex task requires a sophisticated neural network, which contains a large number of model weights.
Meanwhile, the range of each weight is also wider in the complex task.
In addition, Figure~\ref{fig:budget} (a-c) shows the accuracy of \system\ increases with the number of clients. This matches our observations in the previous analysis of bias and variance of \system.


In Table~\ref{table:performance}, we present the accuracy results on MNIST, Fashion-MNIST, CIFAR10 for selected values of $\epsilon$. As illustrated, the training models on MNIST, Fashion-MNIST, and CIFAR10 can achieve a comparable accuracy to the noise-free results after $\epsilon$ is larger than 0.5, 5, 10, respectively.
The accuracy drops to around 10\% accuracy after $\epsilon$ decreases to 0.1 for MNIST, 0.5 for Fashion-MNIST and 1 for CIFAR-10, respectively. This gives a reference of how to select appropriate value for $\epsilon$.
%Due to the larger random noise required by the stronger privacy guarantee, 
%the performance drops to almost 10\%, which is the same as a random guess in these three datasets.
%These results argue that \system\ applies to different privacy requirements. It can effectively improve the performance even when the privacy budget is relatively tight than previous works and other mechanisms. 



\section{Related Work}

Differential privacy \cite{dwork2014algorithmic} has been widely studied in last ten years. For stronger privacy, several local differential privacy mechanisms were proposed, e.g.,~\cite{duchi2013local,duchi2014privacy,erlingsson2014rappor,duchi2018minimax, wang2019collecting}.

Recently, more works studies how to use DP in federated learning \cite{geyer2017differentially,mcmahan2017learning} or use LDP in the federated learning \cite{bhowmick2018protection,nguyen2016collecting,seif2020wireless,truex2020ldp}.
However, existing approaches can not be applied practically on deep learning. 
Some of them \cite{nguyen2016collecting,seif2020wireless} only focus on small tasks and simple datasets and do not support deep learning approaches yet.
The other works \cite{bhowmick2018protection,truex2020ldp} studied the LDP on federated learning problem. However, as we discussed in the experiments part, both of them hardly achieve a good performance with a small limited budget.
Bhowmick et al. \cite{bhowmick2018protection} is the first work focus on the LDP on federated learning with deep learning models. However, it first need a strong assumption that attacker has little prior acknowledge about user data. Meanwhile, it spends $\epsilon = 500$ for MINST and $\epsilon = 5000$ for CIFAR-10, which means the LDP is not practical and needs traditional differential privacy for second protection.
Last, they did not report the absolute performance on MNIST and CIFAR-10. 
Truex et al. \cite{truex2020ldp} is another recent work. It uses It contains two obvious problems. First, it replaces LDP by Condensed LDP (CLDP), which spends a large privacy budget $\epsilon$ with a large clip bound reported in the work. Second, this work does not provide a complete privacy utility analysis of the number of weights and communication rounds.
Due to the high variance of the noises in their approaches, it requires more communication rounds between cloud and clients, which spends more privacy cost in their framework.
Our approach focus on solving the weakness of all previous approaches and accelerates the practical solution on complex dataset.

Besides FL communication framework, there are other communication frameworks with differential privacy protection, such as teacher-student communication \cite{papernot2017semi,papernot2018scalable}. The teacher models are fixed model who want to privately transfer their knowledge to the student side, which is very different to FL communication. So, we do not compare them in this paper.




\section{Conclusion}
In this paper, we propose a new mechanism for LDP, show how to apply it to protect federated learning, and apply splitting and shuffling mechanism to each local clients’ gradients to mitigate the privacy degradation caused by high data dimension and many query iterations.
Our empirical studies demonstrate the proposed system performs better than previous related works on the same image classification tasks. Hopefully, our work can considerably accelerate the practical applications of LDP in federated learning.

% In the future, several research topics can be further explored, such as preventing client anonymization from side-channel attacks, designing a better data perturbation mechanism, and applying the proposed mechanism to natural language processing, speech recognition or graph learning. Moreover, it is of profound significance to generalize the proposed privacy-preserving techniques to other scenarios.

==> pairwise_results.tex <==
\begin{table}[htbp]
\centering
\caption{Pairwise PPMI in Accuracy and AUC (mean $\pm$ std)}
\label{tab:exp}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Model & AUC   \\ \hline
MVGCN & 94.74$\pm$5.62 \\ \hline
EA-MVGCNNs & 97.71$\pm$4.73  \\ \hline
EA-MVGCNs &  97.83$\pm$4.59 \\ \hline
\end{tabular}
\end{table}

==> tab_dataset.tex <==
\begin{table}[t]
% \scriptsize
\centering
\caption{Basic statistics of datasets}
\label{tab:dataset}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{cccccc}
\toprule
\textbf{Dataset} & \textbf{\# Sample} & \textbf{\# View} & \textbf{\# Feature} & \textbf{\# Class} & \textbf{\# Instrument}\\
\hline
HIV      & 70  & 2  & 90 $\times$ 90   & 2 & fMRI \& DTI \\
BP       & 97  & 2  & 82 $\times$ 82   & 2 & fMRI \& DTI \\ 
PPMI     & 754 & 6  & 84 $\times$ 84   & 2 & DTI\\
\bottomrule
\end{tabular}
}
\end{table}

==> tab_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\centering
\caption{Classification results in Accuracy and AUC (mean $\pm$ std)}
\label{tab:exp}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Datasets} & \multicolumn{2}{c|}{HIV}         & \multicolumn{2}{c|}{BP}           & \multicolumn{2}{c|}{PPMI}       \\ \cline{2-7} 
                          & Accuracy       & AUC             & Accuracy        & AUC             & Accuracy       & AUC            \\ \hline
SingleBest                & 80.11$\pm$6.84 & 81.73$\pm$6.93  & 82.55$\pm$6.32  & 83.70$\pm$6.93  & 70.47$\pm$4.39 & 71.47$\pm$4.71 \\ \hline
3D-CNN                    & 50.17$\pm$8.48 & 50.94$\pm$9.83  & 47.94$\pm$10.41 & 48.49$\pm$12.83 & 49.62$\pm$8.48 & 50.05$\pm$9.43 \\ \hline
MVCNN                     & 48.39$\pm$8.34 & 49.11$\pm$9.27  & 49.73$\pm$8.99  & 50.38$\pm$9.48  & 50.57$\pm$4.61 & 51.06$\pm$6.17 \\ \hline
MVGCN                     & -              & -               & -               & -               & 73.91$\pm$7.19 & 74.65$\pm$8.94 \\ \hline
E-MVGCN                   & 75.59$\pm$7.52 & 77.01$\pm$ 8.94 & 77.73$\pm$7.04  & 78.94$\pm$8.51  & 74.23$\pm$7.33 & 75.69$\pm$9.91 \\ \hline
E-GCNNs                   & 84.70$\pm$7.91 & 85.68$\pm$9.47  & 86.23$\pm$5.71  & 87.48$\pm$7.51  & 75.63$\pm$5.91 & 76.63$\pm$7.18 \\ \hline
E-GCNs                    & 84.19$\pm$6.94 & 85.93$\pm$7.42  & 86.54$\pm$5.59  & 87.76$\pm$8.17  & 76.97$\pm$5.37 & 77.66$\pm$7.48 \\ \hline
EA-GCNNs                  & 86.84$\pm$7.19 & 87.14$\pm$8.66  & 88.59$\pm$5.21  & 89.43$\pm$6.11  & 85.36$\pm$3.79 & 86.18$\pm$5.36 \\ \hline
EA-GCNs                   & 87.65$\pm$8.85 & 87.94$\pm$9.97  & 87.16$\pm$4.74  & 88.93$\pm$7.15  & 84.28$\pm$3.61 & 85.47$\pm$6.54 \\ \hline
\end{tabular}
\end{table*}



% \begin{table*}[htbp]
% \centering
% \caption{Classification results in Accuracy and AUC (mean $\pm$ std)}
% \label{tab:exp}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% Datasets                      & HIV   & HIV                          & BP      & BP                                  & PPMI      & PPMI                            \\ \hline
% SingleBest & 80.11$\pm$6.84    &  81.73$\pm$6.93  &   82.55$\pm$6.32  &   83.70$\pm$6.93 & 70.47$\pm$4.39 & 71.47$\pm$4.71 \\ \hline
% DuSK                          &                                      &                                     &                                     \\ \hline
% KSTM                          &                                      &                                     &                                     \\ \hline
% 3D-CNN          &  50.17$\pm$8.48       &   50.94$\pm$9.83         &       47.94$\pm$10.41 &  48.49$\pm$12.83 & 49.62$\pm$8.48  &  50.05$\pm$9.43                    \\ \hline
% MVCNN             &  48.39$\pm$8.34       &   49.11$\pm$9.27         &    49.73$\pm$8.99     &  50.38$\pm$9.48    & 50.57$\pm$4.61  &   51.06$\pm$6.17                 \\ \hline
% MVGCN           & -   & - & - &  -  & 73.91$\pm$7.19     &   74.65$\pm$8.94               \\ \hline
% E-MVGCN         & 75.59$\pm$7.52   &  77.01$\pm$ 8.94 & 77.73$\pm$7.04 &  78.94$\pm$8.51     & 74.23$\pm$7.33     &  75.69$\pm$9.91                \\ \hline
% E-GCNNs                       & 84.70$\pm$7.91  &  85.68$\pm$9.47                    & 86.23$\pm$5.71  &  87.48$\pm$7.51                & 75.63$\pm$5.91 & 76.63$\pm$7.18                      \\ \hline
% E-GCNs                        & 84.19$\pm$6.94  &  85.93$\pm$7.42                     & 86.54$\pm$5.59  & 87.76$\pm$8.17   &   76.97$\pm$5.37 & 77.66$\pm$7.48 \\ \hline
% EA-GCNNs                      & 86.84$\pm$7.19 &  87.14$\pm$8.66                   & 88.59$\pm$5.21 &  89.43$\pm$6.11                  & 85.36$\pm$3.79  &  86.18$\pm$5.36                             \\ \hline
% EA-GCNs                      & 87.65$\pm$8.85  &87.94$\pm$9.97                    & 87.16$\pm$4.74 &  88.93$\pm$7.15                  & 84.28$\pm$3.61  &  85.47$\pm$6.54                 \\ \hline
% \end{tabular}
% \end{table*}
